Neural Splines: Fitting 3D Surfaces with Infinitely-Wide Neural Networks

We present Neural Splines, a technique for 3D surface reconstruction that is based on random feature kernels arising from infinitely-wide shallow ReLU networks. Our method achieves state-of-the-art results, outperforming recent neural network-based techniques and widely used Poisson Surface Reconstruction (which, as we demonstrate, can also be viewed as a type of kernel method). Because our approach is based on a simple kernel formulation, it is easy to analyze and can be accelerated by general techniques designed for kernel-based learning. We provide explicit analytical expressions for our kernel and argue that our formulation can be seen as a generalization of cubic spline interpolation to higher dimensions. In particular, the RKHS norm associated with Neural Splines biases toward smooth interpolants.

==> 07b_broader.tex <==
\section*{Broader Impact}

Our work uses kernels that are inspired by neural networks for the task 3D surface reconstruction. While other methods for solving this task exist, our approach improves the current state of the art and could lead to a more effective and widespread use of 3D reconstruction methods in real-life applications. Surface reconstruction is in fact a core technology in a variety of practical domains, including computer aided geometric design (CAGD), robotics, autonomous driving, reverse engineering, architectural analysis, medical imaging, and augmented reality.

While robust, high quality surface reconstruction opens the door to many exciting applications, like any technology, it can be used for nefarious purposes. In particular, as with many advances in imaging, our 3D surface reconstruction method could be used by corporations and governments in surveillance systems deployed without their targets' consent. 


